Tailor: Size Recommendations for High-End Fashion Marketplaces

In the ever-changing and dynamic realm of high-end fashion marketplaces, providing accurate and personalized size recommendations has become a critical aspect. Meeting customer expectations in this regard is not only crucial for ensuring their satisfaction but also plays a pivotal role in driving customer retention, which is a key metric for the success of any fashion retailer. We propose a novel sequence classification approach to address this problem, integrating implicit (Add2Bag) and explicit (ReturnReason) user signals. Our approach comprises two distinct models: one employs LSTMs to encode the user signals, while the other leverages an Attention mechanism. Our best model outperforms SFNet, improving accuracy by 45.7%. By using Add2Bag interactions we increase the user coverage by 24.5% when compared with only using Orders. Moreover, we evaluate the models' usability in real-time recommendation scenarios by conducting experiments to measure their latency performance.

==> code/pmcv_hyperparameters.tex <==
\begin{lstlisting}[style=yaml]
input_hierarchy:
    - ["user_id", "category_id", "brand_id"]
    - ["user_id", "cateogry_id"]
    - ["user_id", "brand_id"]
    - ["user_id"]
    - ["category_id", "brand_id"]
    - ["category_id"]
\end{lstlisting}

==> code/sfnet_hyperparameters.tex <==
\begin{lstlisting}[style=yaml]
user_inputs:
    - "user_id",
product_inputs:
    - "brand_id"
    - "category_id"
    - "scale_id"
    - "product_id"
embedding_dim: 20
user_pathway_dims: [50, 30, 20]
item_pathway_dims: [50, 30, 20]
combined_pathway_dims: [100, 200, 400, 1000]
activation: "tanh"
dropout: 0.05
\end{lstlisting}

==> code/ssp-attention_hyperparameters.tex <==
\begin{lstlisting}[style=yaml]
embeddings_parameters:
  brand_id:
    dim: 64
  category_id:
    dim: 48
  return_reason:
    dim: 2
  size_position:
    dim: 16
  scale_id:
    dim: 48
  event_type:
    dim: 2
TransformerBlock1:
  num_heads: 12
TransformerBlock2:
  num_heads: 16
MLP:
  activation: relu
  dropout: 0.01
  hidden_state_dimensions:
    - 150
    - 100
\end{lstlisting}


==> code/ssp-lstm_hyperparameters.tex <==
\begin{lstlisting}[style=yaml]
embeddings_parameters:
  brand_id:
    dim: 8
  category_id:
    dim: 4
  return_reason:
    dim: 2
  size_position:
    dim: 3
  scale_id:
    dim: 6
  event_type:
    dim: 2
BiLSTM:
  dropout: 0.01
  hidden_layer_size: 25
  number_layers: 2
ProductEncoder:
  activation: relu
  dropout: 0.01
  hidden_state_dimensions:
    - 50
    - 25
MixerEncoder:
  activation: relu
  dropout: 0.01
  hidden_state_dimensions:
    - 150
    - 100
\end{lstlisting}
